Renormalization and Coarse-graining of Loop Quantum Gravity

The continuum limit of loop quantum gravity is still an open problem. Indeed, no proper dynamics in known to start with and we still lack the mathematical tools to study its would-be continuum limit. In the present PhD dissertation, we will investigate some coarse-graining methods that should become helpful in this enterprise. We concentrate on two aspects of the theory's coarse-graining: finding natural large scale observables on one hand and studying how the dynamics of varying graphs could be cast onto fixed graphs on the other hand. To determine large scale observables, we study the case of hyperbolic tetrahedra and their natural description in a language close to loop quantum gravity. The surface holonomies in particular play an important role. This highlights the structure of double spin networks, which consist in a graph and its dual, which seems to also appear in works from Freidel et al. To solve the problem of varying graphs, we consider and define loopy spin networks. They encode the local curvature with loops around an effective vertex and allow to describe different graphs by hidding them in a coarse-graining process. Moreover, their definition gives a natural procedure for coarse-graining allowing to relate different scales. Together, these two results constitute the foundation of a coarse-graining programme for diffeomorphism invariant theories.

==> CHANGES <==
Changes in version 4.2 (September 2015)
o Fixed issue between titlesec and tocloft regarding
  part numbering in the ToC (classicthesis.sty). 
	Thanks to Enrico Gregorio and Henri Menke.
o Fixed bug with colored lines and graffiti 
  (classicthesis.sty). Thanks to Enrico Gregorio and
  Stefano Bragaglia for the fix! (Also switched
  graffiti from \slshape to \itshape.)
o Changed \vspace*{8ex} to \vspace{8ex} (Contents.tex)	
o Moved \cleardoublepage from end of Contents.tex 
  to appropriate position in ClassicThesis.tex
o \bflabel of acronym package removed, as it was 
  removed from acronym package and caused errors.
  Now set \aclabelfont to \acsfont for consistency.
o Converted major files to UTF-8 (thanks to Jörn Hees)
  (Bibliography.bib excluded for now as BibTeX cannot
  handle UTF-8)
o Added support for BibLaTeX in 
  classicthesis-config.tex and Bibliography.tex
	(thanks to Jörn Hees).
	For LyX we will have a work-around for testing.
o Added an example for one's own publication list
  (via BibLaTeX) in Publications.tex (renamed from 
	Publication.tex)
o Replaced/updated scrpage2 with scrlayer-scrpage 
  in classicthesis.sty (thanks to Ivo Pletìkosić).
X Worked on Appendix case with floatperchapter 
  (works for captions but not for references so far)
	Thanks to Claus Lahiri and Clemens Niederberger 
	for their help on this.
	[REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]	
X Removed fixltx2e from classicthesis-config.tex and
  have classicthesis.sty use or emulate the latest 
	LaTeX kernel via latexrelease (option: latest)
  (thanks to Jörn Hees).
	[REMOVED AS IT IS NOT AVAILABLE IN MANY 
	DISTRIBUTIONS, SEE ISSUE #107]
	
Changes in version 4.1 (August 2012)
o Working towards XeLaTeX support:
	- "ifxetex" package for checking whether
	  XeTeX is in use (classicthesis.sty)
	- Adjusted part, chapter, and tocEntry 
	- Thanks to Joerg Weber for his ideas and code
	- Option "pdfspacing" does not work for XeTeX
	  and is disabled when XeTeX is running
	  (maybe implement spacing with fontspec later)
o Load additional packages in order to 
  reduce warnings (classicthesis-config.tex)
	- "textcomp" to fix warnings with missing font 
	  shapes
	- "scrhack" to fix warnings when using KOMA 
	  with listings package  
o Replaced \mathrm-command with \textrm-command
  (Chapter03.tex)

Changes in version 4.0 (December 2011)
o Due to lots of issues and complaints, 
  classicthesis-preamble.sty is replaced by 
  classicthesis-config.tex (which is cleaner,
  nicer, better, etc. than before!)
o No per-chapter-numbering also for equations 
  (classicthesis.sty and Chapter03.tex)
o classicthesis.sty now also works without the 
  KOMA-classes (scrbook, scrartcl, etc.):
	- This affects the text body shape, where the
	  package "typearea" is always loaded in order 
	  to use \areaset
	- And affects the layout of footnotes where the 
	  package "footmisc" is loaded otherwise
	  (not 100\% identical look-and-feel but OK)
o Help for using spanish babel with classicthesis 
  (classicthesis-config.tex)
o Note about pdfsync issues with graffiti 
  (Chapter01.tex)
o Minor clean-up of comments and duplicate lines 
  (classicthesis.sty)
o Adjusted the colophon text (Colophon.tex)
o Increased space for labels in the LoF, LoT, LoL
o Included version information on the title page and
  in the drafting and final version information 
  (classicthesis.sty and Titlepage.tex)

Changes in version 3.0 (June 2011)
o There have been some major changes in order to port 
  classicthesis to LyX easily. See below for details.
  Special thanks go to Ivo Pletikosi\'c for all his 
  hard work he put into this project!
o Changes in ClassicThesis.tex:
	- Redundant fleqn removed from documentclass options 
	 (will be set by amsmath package in preamble)
	- KOMA adjustments for documentclass: 
	  fontsize=11pt,paper=14
	- Moved language options into documentclass due to LyX
	  issues with babel
o Changes in classicthesis.sty:
	- Removed bcor from \areaset command so that it can
	  be set via \documentclass option (BCOR=)
	- New \ctparttext command for putting preamble text
	  after part titles (see ClassicThesis.tex for examples)
	- \graffito command now also available as original
	  \marginpar (backward compatibility is enabled)
	- Chapter number in margin done with \oldmarginpar
o Changes to classicthesis-preamble.sty:
  - Fixed autoref for subfigures (see Chapter 2 for example)
  - Fixed issues with redefining autoref strings (for
      different languages)
	- Now contains all configuration information, such as
	  the title, your name etc.
	- This package now also loads classicthesis.sty, change
	  the options classicthesis to be loaded with here  
	- Package inputenc now loaded with latin9 option 
	- Package listings now also loaded here
	- Now safer package loading regarding options by
	  using \PassOptionsToPackage command extensively
	- Inserted new string for \mySubtitle
o Changes in Titlepage.tex and Titleback.tex because of new 
  string \mySubtitle
o Changed a lot of the documentation, e.g., in Chapter01.tex

Changes in version 2.9 (January 2011)
o Fixed onlytext euler font for MinionPro font (in 
  classicthesis.sty)
o Option "listsseparated" deprecated, because it led to some
  strange side-effects (in classicthesis.sty)
o Changed default font size to 11pt (in ClassicThesis.tex) and
  adjusted text block size accordingly (in classicthesis.sty)
o Fixed bug with backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o New option "floatperchapter" for classicthesis.sty, removed 
  all code for that from classicthesis-ldpkg.sty
o Removed "nochapters" option from classicthesis-ldpkg.sty
o Removed redundant loading of listings package (in
  classicthesis-ldpkg.sty)
o Fixed some headline bug in example classicthesis-book.tex
o Fixed a bug when using parts with plain latex as in example
  classicthesis-book.tex (in classicthesis.sty)

Changes in version 2.8 (March/May 2010)
o Fixed serious \graffito bug in classicthesis.sty
  (thanks to Lorenzo Pantieri and Enrico Gregorio)
o Included backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o Fixed drafting issues (draft information not shown at all)
  caused by wrong code for listings and listsseparated options
  in classicthesis.sty 

Changes in version 2.7 (February 2010, cumulative release)
o Removed option for classicthesis-ldpkg.sty: nobackref 
  Introduced instead option "backref" for consistency
  which works the other way (no backrefs by default)
  
Changes in version 2.6.2 (January 2010, released as beta)
o New option for classicthesis-ldpkg.sty: nobackref 
  (removes links to cited page in bibliography)
o Fixed some spacing issues for LoF, LoT, LoL with option
  "listsseparated" (in classicthesis.sty)

Changes in version 2.6.1 (October 2009, released as beta)
o Removed \myChapter and \myPart, you can now use the regular
  \chapter and \part commands (in classicthesis.sty)
  (thanks to Hinrich Harms for this)
o Fixed used KOMA-options: numbers=noenddot, cleardoublepage=empty
  (in ClassicThesis.tex)
o Included hack to use citations in float environments, will 
  be fixed with caption package version 3.2 (in classicthesis.sty)
o Included some font and text area fine-tuning code 
  (in ClassicThesis.tex)
o Some testing with Libertine font (classicthesis-book.tex)
o Fixed numbering of listings used in different chapters
  (in ClassicThesis.tex, classicthesis.sty, classicthesis-ldpkg.sty)
o Spacing between listings in different chapters and after List 
  of Listings header fixed (in classicthesis.sty)
o Increased \newnumberwidth to sizeof(999) which is better for 
  documents with more than 99 pages (in classicthesis.sty)
o New option for classicthesis.sty: manychapters
    
Changes in version 2.6 (August 2009)
o Centered the title page with the addmargin environment
  (thanks to Nicolas Repp for the hint)
o Fixed header for page two of Table of Contents (with 3 
  or more pages) (in Contents.tex)
o Added numbering of \subsubsection (in Contents.tex)
o Added correct Table of Contents entries for \subsubsection
  (in classicthesis.sty)
o Added printonlyused option to loading acronym package
  (in classicthesis-ldpkg.sty)
o Some code for "clean" hyperlinks (w/o color and w/o boxes)
o Minor fix for \graffito (in classicthesis.sty)

Changes in version 2.5.1 (May 2009, released as beta)
o New option for classicthesis.sty: dottedtoc
  (Refer to the manual for more information.)
o New option for classicthesis.sty: listings
  (Refer to the manual for more information.)
  (Credit + thanks to Prof. Enrico Gregorio)
o Minor clean-up and bug-fixing

Changes in version 2.5 (October 2008, cumulative release)
o Increased text-width for better page layout (experimental)
o Cumulative release, some minor clean-up and bug-fixing

Changes in version 2.4.{1--3} (February and April 2008,
released as betas)
o Switched back to "obsolete" KOMA options due to 
  compatibility issues on some installations
o Increased robustness of \cauthor command in 
  classicthesis-ldpk.sty
o Spacing fix for \sectionmark (in classicthesis.sty) 
o Made Booleans private (in classicthesis.sty)
o Acronyms header for long acronym lists (in Contents.tex)
o Moved "amsmath" package from classicthesis.sty to
  ClassicThesis.tex
o "MinionPro" package now loaded with "mathlf" option
  instead of "osf" option (in classicthesis.sty)
o Fixed issue with contents headings (in classicthesis.sty
  and in Contents.tex)
o Thanks to Lorenzo

Changes in version 2.3 (November 2007)
o Fixed serious bug with \myChapter command (using plain 
  LaTeX)
o Removed hypcap package from classicthesis-ldpkg.sty and
  placeins package from classicthesis.sty. Put both into
  ClassicThesis.tex for finer end-user control
o Removed obsolete KOMA options from ClassicThesis.tex
o Option "subfigure" deprecated, replaced by "subfig" (in 
  classicthesis.sty)
o Inserted some mechanisms to detect whether subfig(ure) 
  package was loaded or not (in classicthesis.sty)
o Inserted some mechanism to detect whether classicthesis
  packackage was loaded or not (in classicthesis-ldpkg.sty)
o Moved "headlines" code block a bit up in 
  classicthesis.sty (seemed to cause problems with new
  KOMA-Script classes)
o Removed accidental "natbib" from classicthesis-ldpkg.sty  
o Some fine-tuning in (Dirty)Titlepage.tex
o Thanks to Lorenzo and Denis! :-)

Changes in version 2.2 (October 2007)
o \myChapter and \myPart now take an optional argument
  just as the regular \part and \chapter commands
o Did some minor changes to classicthesis-book.tex
  so it's a better example
o Inserted some \cleardoublepage before \myPart 
  occurences to avoid pdfbookmark problems
o Introduced some general typographic fine-tuning
  (linespread, penalties, etc.)
o Did some fine-tuning of the \graffito command

Changes in version 2.1 (July 2007)
o Removed duplicate xcolor package call from 
  classicthesis-ldpkg.sty and shifed some color
  definitions around
o Removed re-definition of \ttdefault

Changes in version 2.0 (June 2007, cumulative release)
o Better setup of the list of acronyms 
  (in classicthesis-ldpkg.sty)
o Using KOMA option footinclude in ClassicThesis.tex
  (text block sizes are adjusted to this)
o New option for classicthesis.sty: minionpro
o New option for classicthesis.sty: minionprospacing
o New option for classicthesis.sty: pdfspacing
  (Refer to the manual for more information.)

Changes in version 1.7 (May 2007, not released separately)
o Removed \graphicspath from ClassicThesis.tex
o Use the nag package to ensure "compliance"
o Switched from ccaption to caption in classicthesis-ldpkg.sty
  (setup via \captionsetup in ClassicThesis.tex)
o Switched from subfigure to subfig in classicthesis-ldpkg.sty
o Removed obsolete "usenames" option from loading xcolor package
o Noticed problem with \thelstlisting on some installations
  (commented out in classicthesis-ldpkg.sty)
o Noticed problem with some hyperlinks on some installations
  (could not determine cause)

Changes in version 1.6 (April 2007, not released separately)
o Included greetings to Lorenzo Pantieri for many very useful
  suggestions
o Introduced new commands in classicthesis-ldpkg.sty to make
  adaptation of backrefs to different languages easier
   - \backrefnotcitedstring (ref is not cited)
   - \backrefcitedsinglestring (ref is cited on one page)
   - \backrefcitedmultistring (ref is cited on multiple pages)
o Removed ellipsis package from classicthesis-ldpkg.sty due to 
  some undesired results for some users
o Removed the following packages from classicthesis-ldpkg.sty as 
  these seem to require changes to their options from most users:
  inputenc, babel, natbib (now in ClassicThesis.tex)
o New option for classicthesis-ldpkg.sty: nochapters
  Use the package with classes that do not have chapter divisions 

Changes in version 1.5 (April 2007, not released separately)
o Fixed some bugs to use classicthesis.sty for article layout
o Inserted some info/warnings when using nochapter/parts
o Extended the manual: examples for using classicthesis.sty for
  other projects than a thesis (source available in folder
  "Examples")
o Some minor adjustments in classicthesis-ldpkg.sty
o Fixed some spelling mistakes

Changes in version 1.4.2 (March 2007)
o Renamed loadpackages.sty to classicthesis-ldpkg.sty due to
  TeX Live package tree issues

Changes in version 1.4.1 (March 2007)
o Fixed some wording concerning the license :-o
o Added fixltx2e and ellipsis packages to to loadpackages.sty to correct
  some minor glitches
o Fixed and changed some things about ToC entries of parts
o Some minor bug fixes

Changes in version 1.4 (January 2007)
o Replaced \lineheight with \baselineskip in classicthesis.sty
o Removed obsolete "usenames" option from xcolor package (classicthesis.sty)
o Now classicthesis.sty processes the global a5paper option and adjusts 
  the layout accordingly (experimental!)

Changes in version 1.3.1 (August 2006)
o Urgent bug concerning ToC spacing etc. fixed

Changes in version 1.3 (August 2006) 
o New option for classicthesis.sty: parts
  Turn this on if you use Part divisions. It fine-tunes the ToC and
  adds support for Part division via \myPart{} (cf. \myChapter{})
  (The style of this feature is preliminary, any suggestions?!)
o New option for classicthesis.sty: eulermath
  Uses the awesome Euler fonts for math (Palatino fonts are default).
o Added mparhack package to loadpackages.sty to get the graffiti right
o Added a hint to loadpackages.sty on how to typeset the List of 
  Listings consistently with classicthesis
o Some minor fine-tuning of typographic details
o Collaboration with babel package improved (now easier to use
  with other languages than English)
o Added appropriate textwidth values for 11pt Palatino and Minion
  (See comments near \areaset in classicthesis.sty)
o Note: There is a problem with the case of math text in part-, 
  chapter-, and section titles and I have no clue how to fix this 
  (either the case or the spacing breaks). So far, I chose the case. :-(

Changes in version 1.2 (June 2006)
o Setup a little postcard collection: http://postcards.miede.de
o Changed stupid spelling mistake: "A Homage" => "An Homage" D'oh!
o New option for classicthesis.sty: nochapters
  Allows to use the look-and-feel with classes that do not use chapters.
o New option for classicthesis.sty: beramono
  Loads Bera Mono as typewriter font. (Default = no typewriter font.)
o Included list of files, see LISTOFFILES.  

Changes in version 1.1 (May 2006)
o classicthesis.sty now stand-alone and usable w/o whole bundle!
o classicthesis.sty compatible with both LaTeX and PDFLaTeX
  Note: this is only true for classicthesis.sty, not the whole bundle.
o New option for classicthesis.sty: subfigure
  Tells the style to add the respective option when loading tocloft.
o Now loading microtype package w/o options (classicthesis.sty)
o Fixed overfull hbox warnings for ToC entries (classicthesis.sty)
o No longer depending on a particular caption package (classicthesis.sty)
o Layout for subsubsections provided (classicthesis.sty)
o PDF opens on title page (ClassicThesis.[tex|pdf])
o Files are a bit more "ASCII-friendly" (all)
o Note: Thanks to all the folks who already sent me a postcard! :-)

Version 1.0 (March 2006)
o First public release

==> Chapters/save_Chapter10.tex <==
%*****************************************
\chapter{The renormalization of the Immirzi parameter} \label{ch:Immirzi}
%*****************************************

\inspiquote{Do what I do. Hold tight and pretend it’s a plan!}{The Doctor}

In this chapter, we will stand a bit astray of the full thesis plan. Indeed, in the last two chapters, we consider the definition of normals for hyperbolic tetrahedra. This led us to consider connections on the hyperboloid or even on the plane that looked like the Ashtekar-Barbero connection. In particular, we saw that some periodicity, due to the compactness of $\mathrm{SU}(2)$, appears in the normals and can lead to problem for reconstruction. The same phenomenom appears with the usual Ashtekar-Babebero connection and we wish to comment on this fact and consider how this might impact the coarse-graining scheme.

In essence, what we aspire to show is that the choice of variables for \ac{LQG}, because the gauge group is non-compact, might be important. Note however that though this problems appear in 3+1D with the Immirzi parameter, it is not confined to this case. In particular, the very same problem can appear in self-dual \textit{euclidean} gravity which has a compact gauge group also. Through a very simple calculation, we will show that a given holonomy cannot resolve all possible curvatures.

This is a not a problem \textit{per se}, since it only means that for high curvature several holonomies are needed. It seems however to have implications with regard to two points. First, this upper bound on the curvature might be what makes the theory finite. Because the Immirzi parameter seems sometimes \textit{ad hoc}, this might triggers discussions on the physicality of all this. Of course, it is also totally possible to believe that it is precisely the Immirzi parameter which saves the day. Second, this will be a problem when coarse-graining as we want to consider larger and larger holonomies. If this is done naively, this might lead to a faulty theory. Naively, we might then expect some kind of \textit{renormalization} of the Immirzi parameter. It may be plausible from a quantum field theory perspective (afterall the Immirzi parameter is a parameter of the theory) as considered in \cite{Benedetti:2011yb}. This is also difficult to make precise as the Immirzi parameter appears in the definition of the gauge structure. This is why we will consider how this problem is solved in \ac{LQC} (as was advertised in chapter \ref{ch:LQC}). In particular, we will see how the problem can be solved in toy models of \ac{LQG} which are designed to reproduce \ac{LQC}.

This chapter is inspired from work in \cite{Charles:2015rda}. It is organized as follows: in a first section, we will restate the results of \cite{Charles:2015rda} and comment on them, in particular on their \textit{would-be} consequences on the renormalization flow. In a second section, we will consider a very simple model of quantum cosmology. The goal is to give the necessary information for the last section which consider how the problems is lifted, within this model, to reproduce \ac{LQC}, which is arguably a caorse-grained theory.

%*****************************************

\section{The Immirzi parameter as a cut-off}

In \ac{LQG}, the Immirzi parameter $\beta$ plays a crucial role. It can be seen as a new coupling constant entering the Palatini action for general relativity in front of an almost-topological term \cite{Holst1996}. But, at a deeper level, it implements a canonical transformation from the original complex self-dual Ashtekar connection, which we will call $\mathcal{A}$, and the real Ashtekar-Barbero $\mathfrak{su}(2)$-connection $A$ \cite{Rovelli:1997na}. This allowed both to work with a compact gauge group $\mathrm{SU}(2)$ (instead of the non-compact Lorentz group $\mathrm{SL}(2,\mathbb{C})$) and to avoid the issue of the reality conditions\footnote{As the Ashtekar connection $\mathcal{A}$ is complex and is thus not equal to its complex conjugate, it can not be simply quantized as a multiplicative operator if the scalar  product   is simply defined by the Gaussian measure. One needs to modify in a non-trivial way either the scalar product or the action of the connection operator (see e.g. \cite{Soo:2001qf}).}. At a more effective level, it enters the \ac{LQG} dynamics in a non-trivial way and seems to be a crucial parameter in the description of quantum black holes (see the review \cite{G.:2015sda}). It also appears to control the couplings to fermionic field and possible quantum gravity induced CP violation \cite{Perez:2005pm, Freidel:2005sn, Mercuri:2006um,Mercuri:2006wb}. The main drawback of the Immirzi parameter is that the fact that Ashtekar-Barbero connection is not a space-time connection anymore and the resulting apparent loss of covariance \cite{Alexandrov2002a} (see also the more recent \cite{Geiller:2012dd,Achour:2013gga}). Nevertheless, this does not cause any problem in practice and one can perfectly define the kinematical Hilbert space of the theory and transition amplitudes between spin network states either by a canonical Hamiltonian \cite{Thiemann:1996aw,Bonzom:2011jv} or by a spinfoam path integral amplitude \cite{Engle:2007wy}. It can however be tempting to go back to the original complex formulation, given by the specific imaginary choice of Immirzi parameter $\beta =\pm i$, and attempt to define an analytic continuation of the real formulation of \ac{LQG} \cite{Achour:2015xga}.

The two important points that we would like to underline in this section are:
\begin{itemize}
\item The connection $A$ is not a space-time connection, except in the special case of the (anti-)self-dual Ashtekar connection ${\cal A}$ for the purely imaginary choice $\beta=\pm i$. It depends on the space-time embedding of the canonical hypersurface $\Sigma$. Considering a Wilson loop $\gamma$, its value will change if we embed it in different canonical space-like hypersurfaces $\Sigma$. This apparently bad feature might be turned into an advantage: it could help us extract a a simpler way the extrinsic data from the Ashtekar-Barbero holonomies and reconstruct the local embedding of the 3d space manifold.

\item The  Ashtekar-Barbero connection, for real $\beta$, is in some sense a projection of the non-compact Lorentz connection into the compact $\mathrm{SU}(2)$ group. We lose some information, due to the periodicity in the extrinsic curvature. At the classical level, different extrinsic curvatures will still lead to the same value of the Wilson loop. This appears to impose a cut-off on the possible excitations of the geometry, more precisely on the extrinsic curvature, i.e. on the speed/momentum of the 3d intrinsic geometry.
\end{itemize}

We will illustrate these two points with the example of a closed loop embedded in space-like hyperboloids with variable curvature within the flat 4d space-time. We will discuss the dependence of the Wilson loop on the curvature of the hyperboloid, to show both how the Ashtekar-Barbero connection depends on the space-time embedding and how we can recover the extrinsic curvature from the value of the holonomy.

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.4]{gfx/hyperboloids.png}
  \caption{\label{fig:plot3d} This shows several hyperboloids of different curvature all containing the same loop in flat spacetime. The curvature of the embedding hyperboloid affects however the curvature of the Ashtekar-Barbero connection.}
\end{figure}

The hyperboloid has been defined in the previous chapter. We can consider a slight generalization in order to have several different hyperboloids of different curvature. Let us start with  the flat 3+1d Minkowski space-time with signature (-+++) and consider the upper sheet of the space-like hyperboloid,
\begin{equation}
-(t-t_{0})^{2}+(x^{2}+y^{2}+z^{2})=-\kappa^{2},\quad
t\ge t_{0}\,,
\end{equation}
with an arbitrary curvature radius $\kappa>0$ and a possible time shift $t_{0}\in\mathbb{R}$. We would like to look at the Ashtekar-Barbero holonomy around a loop of radius $R$, say
\begin{equation}
\gamma\equiv\{t=T,\,x^{2}+y^{2}+z^{2}=R^{2}\}\,,
\end{equation}
where $T$ and $R$ are arbitrarily fixed.
As illustrated on fig.{\ref{fig:plot3d}}, we embed this loop in the whole family of hyperboloid of arbitrary curvature radius $\kappa$ by adjusting their time shift in terms of $\kappa$,
\begin{equation}
t_{0}=T-\sqrt{R^{2}+\kappa^{2}}\,.
\end{equation}
This setting is very similar to \cite{Samuel:2000ue}, but we extend that calculation explicitly to arbitrary curvature $\kappa$.

\begin{figure}[h]
  \centering
  \includegraphics[scale=0.43]{gfx/WR.pdf}\quad
  \includegraphics[scale=0.43]{gfx/Wkappa.pdf}
  \caption{\label{fig:W}The Wilson loop $W$ plotted in terms of the loop size $R$ (in units of $\kappa$) in the upper graph, and in terms of the curvature radius $\kappa$ (in units of $R$) in the lower graph, both for a Immirzi parameter set to $\beta=1$.}
\end{figure}

All the computations can now be done. We refer the reader insterested in the details to the corresponding paper \cite{Charles:2015rda}. Let's concentrate here on the result. For the holonomy around the loop $\gamma$, we obtain for the spin-1 Wilson loop (for the 3-dimensional representation, where the holonomy is represented as a $\mathrm{SO}(3)$ group element):
\begin{equation}
W_{\kappa}(R)=1+2\cos\left(
2\pi\sqrt{1+(1+\beta^{2})\frac{R^{2}}{\kappa^{2}}}
\right)
\end{equation}
We see a clear dependence of the size of the loop in units of the curvature radius of the hyperboloid, as illustrated on the plots in fig.\ref{fig:W}.

This term further depends on the Immirzi parameter $\beta$. For $\beta^{2}=-1$, this extra term vanishes and we recover $W_{\kappa}(R)=3$, which signals a flat connection. This is indeed the case for the complex (anti-)self dual Ashtekar connection, which is a space-time connection and sees that the initial space-time here is flat. However in general, the Ashtekar-Barbero connection is not flat, even though the space-time is flat, and contains information about the curvature $\kappa$ of the hyperboloid. Thus, we can turn that apparently bad feature that $A$ is not a space-time connection into the advantage that we can retrieve some information about the curvature of the canonical slice from the value of the Wilson loop. Indeed, one can invert the relation above and obtain the dimensionless ratio $\kappa/R$ from $W$.

However, this ratio cannot be fully determined. Indeed, there is some periodicity due to the compactness of $\mathrm{SU}(2)$. In general, we only have:
\begin{equation}
\frac{\kappa^{2}}{R^{2}} = \frac{1+\beta^{2}}{(\varphi+k)^{2}-1},\,\,k\in\mathbb{Z}
\end{equation}
with the angle $\varphi$ given in terms of the Wilson loop by:
\begin{equation}
2\pi\varphi = \cos^{-1}\left(\frac{W-1}{2}\right)\,\,\in[0,\pi]\,.
\end{equation}
Therefore, the curvature is not uniquely fixed but determined up to a period $k\in\mathbb{Z}$.

The periodicity implies an ambiguity in the determination of the curvature from the Wilson loop. One could  decide to take the lowest value of the curvature, i.e the highest value of the curvature radius, typically given by the natural choice $k=1$. But this would mean obviously neglecting the possibility of higher curvature fluctuations. In this sense, we see that fixing a real Immirzi parameter leads to a cut-off in curvature in the context of \ac{LQG}.

This highlights our major difficulty: by approximating the spin network by coarse-grained version of it, we will have access only to small curvature information, due to the compactness of $\mathrm{SU}(2)$. Note here, that even if the problem could be avoided with self-dual variables for instance, it still appears in euclidean quantum gravity or with Yang-Mills theory. A quantum theory of gravity coupled to matter fields will still have this problem if they are Yang-Mills interactions. There is a simple way out as suggested by our paper \cite{Charles:2015rda}: it is to renormalize the Immirzi parameter (or an Immirzi-like parameter), though a precise implementation of it is still missing. This however, will not cover the full scale of the problem as presented here if no such parameter is available. It is then particularly enlightning to consider coarse-grained model in \ac{LQG}. \ac{LQC} in particular should have exactly the same problem. But as can be seen in the theory, the Immirzi parameter is still present and is not set to a particular value, which would be a fixed point of the renormalization process. However, the problem seems to be lurking in with respect to the difference between the $\mu_0$ and the $\overline{\mu}$ scheme. And this is, what we will investigate in the remaining of this chapter.

%*****************************************

\section{The single loop model of cosmology}

Let's now consider a model, using technology from \ac{LQG} which might encode cosmological dynamics. It is inspired from the $\mathrm{U}(N)$ \cite{Borja:2010rc,Borja:2010gn,Livine2013} model but stripped out of all the non-necessary ingredients for our purpose. It is in some sense justified only \textit{a posteriori} after the $\mathrm{U}(N)$ can be devised as a simple model reproducing the same kind of dynamics.

The $\mathrm{U}(N)$ model is a simple model aiming at describing homogeneous and isotropic universes using a fixed graph. The graph has only two vertices linked together by a fixed number of edges. To describe a homogeneous and isotropic universe, this has still too many degrees of freedom. It can be reduced by using the $\mathrm{U}(N)$ action on the vertices. Indeed, each vertex can be endowed with a collection of observables which satisfy a $\mathrm{U}(N)$ algebra. Enforcing that the equality between these observables on the two vertices can be understood as a homogeneity and isotropy condition. Because the constraints are first class, we can study the remaining degrees of freedom by simplectic reduction. The observables have the following action: they carry quanta of surfaces from one edge to the other, conserving the total area separating the two vertices. The simplectic reduction leads then to two degrees of freedom, which are conjugated: the total area (which is conserved under transformation) and the angle of the transforamtion on each link (which is the same on each link between the two vertices when the constraints are imposed).

These two degrees of freedom correspond more or less to the degrees of freedom we are interested in cosmology: the scale factor and its conjugate. They have even a nice correspondance with the variables from \ac{LQC}. Indeed as was presented in the chapter \ref{ch:LQC}, the symmetry reduction of \ac{LQC} using the variables of \ac{LQG} leads to two variables $p$ anc $c$. $p$ is the squared scale factor and $c$ is its conjugate which is linked to (extrinsic and intrinsic) curvature. These are precisely the variables which are uncovered in the $\mathrm{U}(N)$ symmetric model.

This model is effective and would do the work, but we will concentrate on a much simpler model which is sufficient to show our problems. We simply called it the single loop model, as it seems quite fit. Let's consider a single vertex and a single link starting and ending on it, making it a loop. On this graph, we have two variables classically which are conjugated : the area of the transverse surface to the loop and the angle of the rotation along the loop. They are the exact equivalent (up to factors) of the two variables of the $\mathrm{U}(N)$ model and do correspond to the variables of \ac{LQC}. This can be described quantum mechanically by wave functions over $\mathrm{SU}(2)$ which are invariant under conjugation, that is functions of the form:
\begin{equation}
\psi : \mathrm{SU}(2) \rightarrow \mathbb{C}
\end{equation}
such as:
\begin{equation}
\forall h,g \in \mathrm{SU}(2),\ \psi(ghg^{-1}) = \psi(h)
\end{equation}
A natural basis for this space of states is given by the characters of $\mathrm{SU}(2)$ which we will write $\chi_j$ where $j$ is the half-integer labelling representations. Therefore, the state can be written:
\begin{equation}
\psi(g) = \sum_{j \in \frac{\mathbb{N}}{2}} \psi_j \chi_j(g)
\end{equation}
There are natural operators on this space that will nicely do the job as observables for curvature and area. There are the holonomy in the fundamental repressentation and the casimir. We write them as:
\begin{equation}
  \left\{\begin{array}{rcl}
  \hat{\chi} \psi(g) &=& \chi_{\frac{1}{2}}(g) \psi(g) \\
  \hat{C} \psi (g) &=& \sum_{j \in \frac{\mathbb{N}}{2}} j(j+1) \psi_j \chi_j(g)
  \end{array}\right.
\end{equation}
Note that these are not precisely the operators for $p$ and $c$. Apart from ordering ambiguities, $\hat{p}$ is simply linked to the casimir by $\hat{p}^2 = \hat{C}$. But for $c$, there is no well-defined operator. This is precisely the point, as we only want exponentials of the operator to be defined. It is therefore appropriate to think of $\hat{chi}$ as $\cos c$ (the even part of the exponential).

Now, let's forget about the numerical factors. As we saw in chapter \ref{ch:LQC}, the classical hamiltonian for cosmology is (expressed in $p$ and $c$):
\begin{equation}
  H = (pc)^2
\end{equation}
Because $c$ does not exist as an operator, we will need to change the Hamiltonian slightly. The most basic thing to do is to consider:
\begin{equation}
  \tilde{H} = 2 p^2 \left(\cos c - 1\right)
\end{equation}
This corresponds more or less to the $\mu_0$ scheme, which we sadly know to be false. But it has the advantage of being writeable in the model we just exposed. The problem is, we only have access to functions of $c$ of the form $\cos nc$ with $n$ an integer. They correspond to the different representations of the holonomy or, alternatively, to powers of the fundamental one. This is a problem though for the $\overline{\mu}$ scheme. Indeed, as we saw, we need more than just the integer exponentials of the connection but all exponentials for all real values of a prefactor. And this cannot be implemented on our compact configuration space (namely $\mathrm{SU}(2)$).

In a more \ac{LQC} like language, everything is behaving as if we were considering $\mathrm{U}(1)$ as a configuration space rather than $\mathbb{R}_\textrm{Bohr}$. Most operators are not well-defined in this context and more importantly, the conjugate to the volume is not well-defined which is however needed for the $\overline{\mu}$ scheme. In the context of \ac{LQC}, this can be interpreted (as we suggested in the beginning of this chapter) as a varying Immirzi parameter. It should be noted though that this is \textit{not} the conventionnal interpretation. Indeed, usually the geometrical interpretation goes as follows: when the scale factor goes larger, the loops, relative to the size of the universe, actually scales down. Therefore, the connection, which is expressed in the comoving coordinates should scale down accordingly. For the fundamental theory, this means the dynamics should be graph changing and rather than a fixed graph with a compact configuration space on each link. This is precisely the problem we face with coarse-graining and renormalization, here in the redux. The problem is particularly manifest as problems in periodicity. Indeed, all our observables are periodic (due to the compactness of $\mathrm{SU}(2)$) but the observables we'd like for quantum cosmology are non-periodic. This is the natural problem we have to face.

%*****************************************

\section{The $\overline{\mu}$ scheme in a coarse-grained fashion}

Let's consider a simpler problem: let's consider a scalar field in a one dimensionnal space. It can be modeled by a function from $\mathbb{R}$ and valued in $\mathbb{C}$ (if we consider a complex scalar field). A coarse-graining of it could be represented by a function from $\mathbb{Z}$ into $\mathbb{C}$. The relation between the discretization and the continuum theory is left open here. But in principle, something similar to the perfect discretization process \cite{Bahr:2009qc} should give an ideal description of the low energy states of the \textit{continuum} theory. Still, we encounter here a problem similar to the problem described above: because of the discretization, the Fourier space becomes compact and it is now impossible to describe the non-periodic dispersion relations on the Brillouin zone. The problem of compactification appears therefore once more but here in the Fourier space.

Technically, let's note here that the problem is a bit different as this is not a problem of compactness of the \textit{configuration} space, but mathematically, it is quite similar. The problem is also different in that it is related to a discretization problem and not strictly a coarse-graining one. Still, it can be recast in this language in the following manner: let's rather consider one discrete theory (with fields from $\mathbb{Z}$ into $\mathbb{C}$) and a second one but with a length between points doubled (so in a sense with fields from $2\mathbb{Z}$ into $\mathbb{C}$ though of course this changes nothing mathematically speaking). We can consider the coarse-graining problem of going from one scale to the other. Incidently, the fixed points should represent the continuum theory (or at least the low energy states of it).

For a (relativistic) free field, the dispersion relation is:
\begin{equation}
E^2 = p^2 + m^2
\end{equation}
with the usual conventions of $c=\hbar=1$ and where $E$ is the energy and $p$ the momentum. Because our coarse-graining is only spatial, energy is not compactified. But momentum will be. This is a problem however as the dispersion relation is clearly not periodic. Indeed, on a lattice, only periodic function of $p$ will exist, that is only those which depend on $p$ up to $\frac{2\pi}{a}$. This is the equivalent in this simpler setting of our compactification problem. A solution though is to simply concentrate on low energy excitations. Indeed, if we consider momentum that are between $-\frac{\pi}{a}$ and $\frac{\pi}{a}$ they can be described both by the original dispersion relation or by a periodic function. But this requires to concentrate on low energy excitations. It could in principle be possible to extend to higher energies by defining energy \textit{bands} but the praticality does not seem straight forward.

Can we do the same thing for \ac{LQG}? Classically, it is possible, at least in the context of \ac{LQC}. We can start with the $\overline{\mu}$ hamiltonian and expand it in terms of sine and cosine of $c$ as shown here:
\begin{center}
\textbf{TODO:} equations
\end{center}
The low energy limit is here replaced by a low curvature limit: as long as $c$ is small, the expansion will be exact. We are quite lucky here as this is one of the property of the $\overline{\mu}$ scheme: it tends to keep $c$ small. For larger values though, the expansion is not directly usuable, apart maybe from analytical continuations.

What we see here is that the coarse-graining leads to some problems which limit the validity of our expansions. The clear path out is not really straight forward. It might be that changing the Immirzi parameter (in some kind of imitation of the \ac{LQC} framework) would be enough or that some divergent series enables the description through large graphs. But the important point is the following: it is important to understand the role of varying graphs.

Indeed, the problem of how varying graphs enable the right dynamics has been recently in the context of \ac{GFT} \cite{Gielen:2013naa}. This is expressed in the formalism of condensed state where the universe consists of many tetrahedron all in the same state\graffito{Note that these condensed states are not gauge-invariant and this is therefore an approximation.}. The fact that the number of tetrahedron is variable allows the right dynamics of \ac{LQC} to be found \cite{Oriti:2016ueo}. Therefore, our major problem is to encode a varying graphs dynamics. More importantly still, it is paramount to understand how the dynamics of small loops might be encoded in some large structures. This is precisely the subject of study of the next part.

%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************

